Ptychopy: GPU framework for ptychographic data analysis

X-ray ptychography imaging at synchrotron facilities like the Advanced Photon Source (APS) involves controlling instrument hardwares to collect a set of diffraction patterns from overlapping coherent illumination spots on extended samples, managing data storage, reconstructing ptychographic images from acquired diffraction patterns, and providing the visualization of results and feedback. In addition to the complicated workflow, ptychography instrument could produce up to several TB's of data per second that is needed to be processed in real time. This brings up the need to develop a high performance, robust and user friendly processing software package for ptychographic data analysis. In this paper we present a software framework which provides functionality of visualization, work flow control, and data reconstruction. To accelerate the computation and large datasets process, the data reconstruction part is implemented with three algorithms, ePIE, DM and LSQML using CUDA-C on GPU.

==> src/abstract.tex <==
X-ray ptychography imaging at synchrotron facilities like the Advanced Photon Source (APS), involves controlling instrument hardwares to collect a set of diffraction
patterns from overlapping coherent illumination spots on extended samples, managing the data storage, reconstructing ptychographic images from acquired diffraction patterns, providing the visualization of results and feedback for the operation. This brings up the need of developing a flexible, robust and user friendly processing pipeline for ptychography data analysis. Here we present a software framework including visualization tools and ptychography reconstruction module for data stream analysis using GPU.
%During a beamline experiment different scanning strategies can be adopted depending from sample environment conditions, data collection speed, data analysis tools etc. This brings the challenge of developing a flexible, robust and user friendly scan builder.




%Here we present a software framework integrated with visualization tools and ptychographic data reconstruction module. 

%The visualization tools is implemented upon PyQt and the ptychographic reconstruction module is a python library based on ePIE reconstruction algorithm implemented with CUDA.


==> src/intro.tex <==
Beamline at the APS uses X-rays and various detectors, equipment to conduct a series of scan experiments for different purposes, such as fluorescence mapping tomography scan, coherent diffraction imaging (CDI) scan, laue depth reconstruction scan, etc. Among these categories, CDI scan is a very novel lensless technique which uses a coherent beam to determine the structure of a specimen of interest. By recording the diffraction pattern of the coherent beam diffracted off the sample, the structure of a specimen of interest can be reconstructed using an iterative phase retrieval algorithm. 

Ptychography~\cite{hoppe1969beugung,faulkner2004movable} is a scanning version CDI method introduced by Hoppe~\cite{hoppe1969beugung}, which is capable of producing high resolution images on extended object, because of its no optics-imposed limits feature on collecting large scatter angle diffraction patterns. It involves recording a set of diffraction patterns by overlapping the scanning illumination spots to image extended, non-isolated samples. Because adjacent illumination spots overlap significantly in the object plane, there are redundant information in the object among diffraction patterns, which could be used to reconstruct both object transmission function and probe function.


There are many ptychography phase retrieve methods, such as relaxed averaged alternating reflections (RAAR) algorithm~\cite{luke2004relaxed}, difference map (DM) algorithm~\cite{thibault2009probe,thibault2008high}, hybrid input-output (HIO) algorithm by Fienup~\cite{fienup1982phase},  maximum likelihood (ML) principles~\cite{thibault2012maximum}, ptychographical iterative engine (PIE)~\cite{rodenburg2004phase} , extended ptychographical iterative engine (ePIE) by Maiden~\cite{maiden2009improved}. These methods try to recover the lost phase using a set of diffraction patterns which are got from overlapping an illumination function through sample. In this paper, we use the ePIE algorithm with Compute Unified Device Architecture (CUDA) implementation introduced in our previous work~\cite{nashed2014parallel} as the reconstruction algorithm. 

Due to the need of higher resolution, brighter light sources, higher throughput of the faster detectors, the size of the resulting ptychography datasets are increasing rapidly. GPU can accelerate image processing and has been used for speeding up data processing, reconstruction~\cite{yue2015accelerating} at the APS. In order to reconstruct the large size datasets, a multi-GPUs based ePIE algorithm is presented in the paper ~\cite{nashed2014parallel}, which can provide high performance speed up on ptychography reconstruction. However, the program is implemented with CUDA in C++ and not convenient to integrate with python environment for the streamlined ptychography. Therefore, we convert the CUDA algorithm to a CPython module which has a python interface to integrate with beamline control, data collecting, storage and visualization.

In addition to ptychography reconstruction, we use PyEpics for controlling the beamline instrument and collection the data. PyEpics~\cite{newville2014pyepics} is a python module which provides python interface for the Experiment Physics and Industrial Control System (EPICS) library. The frontend module for visualization and parameter configuration is implemented with PyQt5. There are also modules that can manage result dataset storage, convert the image format from CSV to other formats such as TIFF, provide feedback to the user about the reconstruction status and result using log file and email. These modules can be easily integrated with ptychography reconstruction module for streamlined data analysis.

There are several software framework that has been developed for handling ptychography scan and data analysis. Nanosurveyor~\cite{daurer2017nanosurveyor} provides a  streamlined processing pipeline to support distributed real-time analysis and visualization of the data for ptychography. The software's backend is based on SHARP (Scalable Hetereogeneous Adaptive real-time Ptychography)~\cite{marchesini2016sharp,shapiro2014chemical}, which uses RAAR as the reconstruction algorithm and running in parallel on multiple graphics processor units (GPUs) in far-field geometry. cSAXS beamline of the Swiss Light Source develops some MATLAB scripts ~\cite{thibault2008high,dierolf2010ptychographic,dierolf2010ptychographic} implementing the DM and ePIE algorithms for the users. PtyPy~\cite{enders2016computational} is a Python open-source software framework featuring clear separation between representations of physical experiments, the models, and the algorithmic implementations to solve the inverse problem. In our previous work ~\cite{nashed2014parallel}, GPU based ePIE and DM phase retrieval algorithms are implemented with CUDA. 
%~\cite{deng2015continuous}~\cite{deng2015simultaneous}


However none of the work mentioned above are using ePIE and DM algorithm running on GPUs as the backend or providing an intuitive customized GUI for the user. The ePIE and DM algorithms running on GPU in our previous work are implemented with C++ and can not easily integrate with other scan modules to form a streamline process pipeline. Plus it does not have an intuitive GUI for accepting information from user and providing feedback. In this paper, a software framework Ptychopy is introduced based on ePIE and DM phase retrieval algorithm with high performance computing backend and a intuitive user interface with customized parameter input and visualization window. The software framework can be running on GPU and integrate with other beamline control and scan packages for streamlined data analysis at the APS. It can also provide functionalities for either real time or off line data analysis and feedback of the result. 


%section{Background}





==> src/ptycho.tex <==


\begin{itemize}
  \item Describe a workflow of the pytcho library, might be better put a workflow image here with a couple lines of illustration
  \item The usage of the pytcho.
  \item The scan challenge due to the rapid changing requirement.
\end{itemize}

==> src/ptychogui.tex <==




%section{Background}

\begin{itemize}
  \item Describe the GUI , functionality of each GUI element.
  \item Workflow design of the software, from how the GUI read the parameters from DMA file and set the parameters.
  \item Snapshot of the GUI interface
  \item Det\_mode ???
\end{itemize}
